Towards VQA Models That Can Read

Studies have shown that a dominant class of questions asked by visually impaired users on images of their surroundings involves reading text in the image. But today's VQA models can not read! Our paper takes a first step towards addressing this problem. First, we introduce a new "TextVQA" dataset to facilitate progress on this important problem. Existing datasets either have a small proportion of questions about text (e.g., the VQA dataset) or are too small (e.g., the VizWiz dataset). TextVQA contains 45,336 questions on 28,408 images that require reasoning about text to answer. Second, we introduce a novel model architecture that reads text in the image, reasons about it in the context of the image and the question, and predicts an answer which might be a deduction based on the text and the image or composed of the strings found in the image. Consequently, we call our approach Look, Read, Reason & Answer (LoRRA). We show that LoRRA outperforms existing state-of-the-art VQA models on our TextVQA dataset. We find that the gap between human performance and machine performance is significantly larger on TextVQA than on VQA 2.0, suggesting that TextVQA is well-suited to benchmark progress along directions complementary to VQA 2.0.

==> sections/old_introduction.tex <==
%%%%%%%%% BODY TEXT
\section{Introduction}

The focus of this paper is endowing VQA models a new ability -- the ability to \emph{read} text in images and answer questions by reasoning over this text.

We have seen tremendous progress in Visual Question Answering (VQA) over the last few years. But one class of questions where all existing VQA models fail catastrophically is the one that requires reading! \devi{cite presentations from VQA challenges}. See Fig.~\ref{fig:teaser}. \devi{Why is this ref not working?} This is surprising because Optical Character Recognition (OCR) is one of the most mature computer vision technologies to date. This is also ironic because among the queries that visually impaired users have for assistive devices -- an application that is often used to motivate VQA -- \emph{frequently} involves questions that require reading to be answered e.g., ``what temperature is my oven set to?'', ``has this medicine expired?'' \devi{cite the original VizWiz paper that introduced the app and had analysis of types of queries users have. Make sure these two examples are representative -- or replace with something else from that paper. Including at least one example question where need to read and then reason on top}. 

One reason why there has been no progress (to the best of our knowledge) on VQA models that can read and reason about text is images is because such questions, while being a dominant category in real applications for aiding visually impaired users, are not popular in standard VQA datasets \devi{cite VQA v1.0, VQA v2.0, Visual7W, etc.}. They do occur frequently in the recent VizWiz dataset~\cite{gurari2018vizwiz} that contains questions asked by visually impaired users on images they took of their surrounding. But the dataset is currently quite small (\devi{list size}). This makes it challenging to study the problem systematically, train effective models, or even draw sufficient attention to this important skill that current VQA models lack. 

To this end, we introduce the \datasetName dataset. It contains \datasetNQuestions{} questions asked by (sighted) humans on \datasetNImages{} images from the Open Images dataset \devi{cite} of categories that tend to contain text e.g., \devi{list a few categories} such that answering the question requires the model to read and reason about text in the image. Each question-image pair has \devi{at least 6} ground truth answers provided by humans. 

Models that do well on this dataset will not only need to parse the image and question as in traditional VQA, but also read the text in the image, identify which of the text might be relevant to the question, and recognize whether some subset of the detected text is directly the answer (e.g., in the case of ``what temperature is my oven set to?'') or additional reasoning is required on the text to answer the question (e.g., ``which team is winning?'').

We propose a new VQA model that includes OCR as a module. We call it \approachName. Our model architecture incorporates the text detected in the image as entities to attend over (in additional to object proposals). It also incorporates the text found in these regions as information (in addition to visual features) that the model learns to reason over. Finally, our model includes a mechanism to decide if the answer produced should be text ``copied'' over from the OCR output (in more of a generation or slot-filling flavor), or should be deduced from the text (in a standard discriminative prediction paradigm popular among existing VQA models). Our model learns this mechanism end-to-end. While currently limited in scope to OCR, our model can be viewed as an initial step towards endowing VQA models the ability to reason over unstructured sources of external knowledge (in this case text found in a test image) and accommodate multiple streams of information flow (in this case predicting an answer from a pre-determined vocabulary or generating an answer via slot-filling). We show that \approachNameShort outperforms strong baselines on our newly proposed \datasetName dataset and is state-of-the-art on the existing VizWiz dataset~\devi{cite}.

%Imagine a household helper robot Alfred. You are away from home and hence ask Alfred to go check if the thermostat has been set to 72 degree Fahrenheit. Alfred is equipped with state of the art navigation and object detection systems powered by deep learning and is able to very quickly get to the thermostat. However, Alfred is unable to do much beyond that because Alfred lacks the capability to recognize and reason about text in the visual world. Given the recent advances in robotics and deep learning, household robots like Alfred are not far off. However for such robots to be really useful, they need to be able comprehend and understand language not only from spoken sources but also visual sources. 


%\marcus{Not sure I would use a robot and navigation example, although we are not doing anything with robots... I think a blind person needing assistance is a closer application?}
%There has been impressive advancement in Optical Character Recognition (OCR) systems over the last few years with systems like \cite{lee2016recursive, he2017multi, gao2017reading, jaderberg2014synthetic} once again powered by deep neural network architectures for both text detection and recognition. While it is necessary to have a good OCR system that alone is not sufficient just like speech recognition alone is not sufficient to build assistants like Alexa and Google Home. Visually grounded robots or assistants like Alfred need to be able to understand and reason about text in the visual world in the context of the task. 



%In this paper, we study this problem in the context of the Visual Question Answering (VQA) task introduced by \cite{antol2015vqa}. Over the years significant progress has been made on the VQA 2.0 dataset with models like Bottom Up Top Down Attention \cite{anderson2017bottom} and Bilinear Attention Networks \cite{kim2018bilinear}. However, these models perform poorly on questions that require image text reading capabilities. The recently released Vizwiz dataset \cite{gurari2018vizwiz} which contains questions directly from blind users provides further motivation to study the problem in more detail - a significant fraction of the questions in the dataset requires OCR and reasoning on it for them to be answered correctly.

Overall, our contributions are 
\begin{itemize}
\item We introduce a novel dataset (\datasetName) containing questions which require the model to read and reason about the text in the image to be answered. 
%We do this because the number of questions which require image text reading and reasoning capabilities is quite limited in the VQA 2.0 and Vizwiz dataset.
\item We propose \approachName: a novel model architecture which explicitly reasons over outputs from an OCR system when answering questions. 
\item \approachNameShort outperforms strong baselines (existing state-of-the-art VQA models) on our \datasetName dataset, and achieves state-of-the-art performance on the Vizwiz dataset.
\end{itemize}



==> sections/results/simple.tex <==
\begin{table}[h]
    \center
    \setlength{\tabcolsep}{12pt}
    \footnotesize
    \begin{tabular}{lllrr}
    \toprule
    \multicolumn{3}{l}{} & \multicolumn{2}{c}{\textbf{Accuracy(\%)}} \\
    \multicolumn{3}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Val}} & \multicolumn{1}{c}{\textbf{Test}} \\
    \midrule
    \multicolumn{3}{l}{\textbf{Q}} & 8.09 & 8.70\\
    \multicolumn{3}{l}{\textbf{I}} & 4.52 & 4.42\\
    \multicolumn{3}{l}{\textbf{O}}& & \\
    \multicolumn{3}{l}{\textbf{I+Q+LA}}& 9.97 & 8.7\\
    \multicolumn{3}{l}{\textbf{I+Q+O+C}}& 17.72 & 18.14\\
    \multicolumn{3}{l}{\textbf{I+Q+O+LA}}& 15.24 & 13.33 \\
    \multicolumn{3}{l}{\textbf{I+Q+O+C+LA}}& 21.50 & 20.87\\
    \multicolumn{3}{l}{\textbf{I+Q+O+C+SA}}& 23.98 & 22.31\\
    
    \bottomrule
    \end{tabular}
    \vspace{0.1cm}
    \caption{Accuracy on \datasetName \marcus{still have to think more about naming}}
    \label{tab:results:ours}
\end{table}

==> sections/results/vizwiz.tex <==


\subsection{Results on Vizwiz}
\begin{table}[t]
    \center
    \begin{tabular}{lllr}
    \toprule
    \multicolumn{3}{l}{\textbf{Model}} & \textbf{Test-Dev Accuracy (\%)} \\
    \midrule
    \multicolumn{3}{l}{\textbf{Question only}} & 36.49\\ 
    \multicolumn{3}{l}{\textbf{Image only}} & 45.43\\
    \multicolumn{3}{l}{\textbf{OCR only}}\\
    \multicolumn{3}{l}{\textbf{OCR max/salient box}}\\
    \multicolumn{3}{l}{} \\
    
    \midrule
    \multicolumn{4}{c}{\textbf{\textit{Without VQA Pretraining}}} \\
    
    \midrule
    \multicolumn{3}{l}{\textbf{Pythia \cite{jiang2018pythia}}}  & 53.41\\
    \multicolumn{3}{l}{\textbf{\textit{~~+ OCR encoding (ours)}}} & 53.72\\
    \multicolumn{3}{l}{\textbf{\textit{~~~~+ Copy mechanism (ours)}}} & 54.13\\
    \multicolumn{3}{l}{} \\
    
    \midrule
    \multicolumn{4}{c}{\textbf{\textit{With VQA Pretraining}}} \\
    \midrule
    
    \multicolumn{3}{l}{\textbf{Pythia \cite{jiang2018pythia}}}  & 54.7\\
    \multicolumn{3}{l}{\textbf{\textit{~~+ OCR encoding (ours)}}} & 54.76\\
    \multicolumn{3}{l}{\textbf{\textit{~~~~+ Copy mechanism (ours)}}} & 53.27\\
    \multicolumn{3}{l}{} \\
    
    \bottomrule
    \end{tabular}
    \vspace{0.1cm}
    \caption{Accuracy on Vizwiz \marcus{still have to think more about naming}}
    \label{tab:results:vizwiz}
\end{table}
